Fairness in Academic Course Timetabling

We consider the problem of creating fair course timetables in the setting of a university. Our motivation is to improve the overall satisfaction of individuals concerned (students, teachers, etc.) by providing a fair timetable to them. The central idea is that undesirable arrangements in the course timetable, i.e., violations of soft constraints, should be distributed in a fair way among the individuals. We propose two formulations for the fair course timetabling problem that are based on max-min fairness and Jain's fairness index, respectively. Furthermore, we present and experimentally evaluate an optimization algorithm based on simulated annealing for solving max-min fair course timetabling problems. The new contribution is concerned with measuring the energy difference between two timetables, i.e., how much worse a timetable is compared to another timetable with respect to max-min fairness. We introduce three different energy difference measures and evaluate their impact on the overall algorithm performance. The second proposed problem formulation focuses on the tradeoff between fairness and the total amount of soft constraint violations. Our experimental evaluation shows that the known best solutions to the ITC2007 curriculum-based course timetabling instances are quite fair with respect to Jain's fairness index. However, the experiments also show that the fairness can be improved further for only a rather small increase in the total amount of soft constraint violations.

==> paper-gnuplottex-fig1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(792,440){\makebox(0,0)[r]{\strut{} 60}}%
      \put(792,769){\makebox(0,0)[r]{\strut{} 80}}%
      \put(792,1097){\makebox(0,0)[r]{\strut{} 100}}%
      \put(792,1426){\makebox(0,0)[r]{\strut{} 120}}%
      \put(792,1754){\makebox(0,0)[r]{\strut{} 140}}%
      \put(792,2083){\makebox(0,0)[r]{\strut{} 160}}%
      \put(792,2411){\makebox(0,0)[r]{\strut{} 180}}%
      \put(792,2740){\makebox(0,0)[r]{\strut{} 200}}%
      \put(924,220){\makebox(0,0){\strut{} 0.91}}%
      \put(1302,220){\makebox(0,0){\strut{} 0.92}}%
      \put(1681,220){\makebox(0,0){\strut{} 0.93}}%
      \put(2059,220){\makebox(0,0){\strut{} 0.94}}%
      \put(2437,220){\makebox(0,0){\strut{} 0.95}}%
      \put(2815,220){\makebox(0,0){\strut{} 0.96}}%
      \put(3194,220){\makebox(0,0){\strut{} 0.97}}%
      \put(3572,220){\makebox(0,0){\strut{} 0.98}}%
      \put(2248,3070){\makebox(0,0){\strut{}comp03}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2585,2567){\makebox(0,0)[r]{\strut{}AMOSA}}%
      \csname LTb\endcsname%
      \put(2585,2347){\makebox(0,0)[r]{\strut{}known best solution}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{paper-gnuplottex-fig1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> paper-gnuplottex-fig2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(792,440){\makebox(0,0)[r]{\strut{} 280}}%
      \put(792,670){\makebox(0,0)[r]{\strut{} 300}}%
      \put(792,900){\makebox(0,0)[r]{\strut{} 320}}%
      \put(792,1130){\makebox(0,0)[r]{\strut{} 340}}%
      \put(792,1360){\makebox(0,0)[r]{\strut{} 360}}%
      \put(792,1590){\makebox(0,0)[r]{\strut{} 380}}%
      \put(792,1820){\makebox(0,0)[r]{\strut{} 400}}%
      \put(792,2050){\makebox(0,0)[r]{\strut{} 420}}%
      \put(792,2280){\makebox(0,0)[r]{\strut{} 440}}%
      \put(792,2510){\makebox(0,0)[r]{\strut{} 460}}%
      \put(792,2740){\makebox(0,0)[r]{\strut{} 480}}%
      \put(924,220){\makebox(0,0){\strut{} 0.82}}%
      \put(1255,220){\makebox(0,0){\strut{} 0.84}}%
      \put(1586,220){\makebox(0,0){\strut{} 0.86}}%
      \put(1917,220){\makebox(0,0){\strut{} 0.88}}%
      \put(2248,220){\makebox(0,0){\strut{} 0.9}}%
      \put(2579,220){\makebox(0,0){\strut{} 0.92}}%
      \put(2910,220){\makebox(0,0){\strut{} 0.94}}%
      \put(3241,220){\makebox(0,0){\strut{} 0.96}}%
      \put(3572,220){\makebox(0,0){\strut{} 0.98}}%
      \put(2248,3070){\makebox(0,0){\strut{}comp05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2585,2567){\makebox(0,0)[r]{\strut{}AMOSA}}%
      \csname LTb\endcsname%
      \put(2585,2347){\makebox(0,0)[r]{\strut{}known best solution}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{paper-gnuplottex-fig2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> paper-gnuplottex-fig3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(792,440){\makebox(0,0)[r]{\strut{} 80}}%
      \put(792,696){\makebox(0,0)[r]{\strut{} 100}}%
      \put(792,951){\makebox(0,0)[r]{\strut{} 120}}%
      \put(792,1207){\makebox(0,0)[r]{\strut{} 140}}%
      \put(792,1462){\makebox(0,0)[r]{\strut{} 160}}%
      \put(792,1718){\makebox(0,0)[r]{\strut{} 180}}%
      \put(792,1973){\makebox(0,0)[r]{\strut{} 200}}%
      \put(792,2229){\makebox(0,0)[r]{\strut{} 220}}%
      \put(792,2484){\makebox(0,0)[r]{\strut{} 240}}%
      \put(792,2740){\makebox(0,0)[r]{\strut{} 260}}%
      \put(924,220){\makebox(0,0){\strut{} 0.8}}%
      \put(1218,220){\makebox(0,0){\strut{} 0.82}}%
      \put(1512,220){\makebox(0,0){\strut{} 0.84}}%
      \put(1807,220){\makebox(0,0){\strut{} 0.86}}%
      \put(2101,220){\makebox(0,0){\strut{} 0.88}}%
      \put(2395,220){\makebox(0,0){\strut{} 0.9}}%
      \put(2689,220){\makebox(0,0){\strut{} 0.92}}%
      \put(2984,220){\makebox(0,0){\strut{} 0.94}}%
      \put(3278,220){\makebox(0,0){\strut{} 0.96}}%
      \put(3572,220){\makebox(0,0){\strut{} 0.98}}%
      \put(2248,3070){\makebox(0,0){\strut{}comp09}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2585,2567){\makebox(0,0)[r]{\strut{}AMOSA}}%
      \csname LTb\endcsname%
      \put(2585,2347){\makebox(0,0)[r]{\strut{}optimal solution}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{paper-gnuplottex-fig3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> paper-gnuplottex-fig4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(792,632){\makebox(0,0)[r]{\strut{} 300}}%
      \put(792,1015){\makebox(0,0)[r]{\strut{} 400}}%
      \put(792,1398){\makebox(0,0)[r]{\strut{} 500}}%
      \put(792,1782){\makebox(0,0)[r]{\strut{} 600}}%
      \put(792,2165){\makebox(0,0)[r]{\strut{} 700}}%
      \put(792,2548){\makebox(0,0)[r]{\strut{} 800}}%
      \put(924,220){\makebox(0,0){\strut{} 0.91}}%
      \put(1302,220){\makebox(0,0){\strut{} 0.92}}%
      \put(1681,220){\makebox(0,0){\strut{} 0.93}}%
      \put(2059,220){\makebox(0,0){\strut{} 0.94}}%
      \put(2437,220){\makebox(0,0){\strut{} 0.95}}%
      \put(2815,220){\makebox(0,0){\strut{} 0.96}}%
      \put(3194,220){\makebox(0,0){\strut{} 0.97}}%
      \put(3572,220){\makebox(0,0){\strut{} 0.98}}%
      \put(2248,3070){\makebox(0,0){\strut{}comp12}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2585,2567){\makebox(0,0)[r]{\strut{}AMOSA}}%
      \csname LTb\endcsname%
      \put(2585,2347){\makebox(0,0)[r]{\strut{}known best solution}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{paper-gnuplottex-fig4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> paper-gnuplottex-fig5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(792,440){\makebox(0,0)[r]{\strut{} 60}}%
      \put(792,769){\makebox(0,0)[r]{\strut{} 80}}%
      \put(792,1097){\makebox(0,0)[r]{\strut{} 100}}%
      \put(792,1426){\makebox(0,0)[r]{\strut{} 120}}%
      \put(792,1754){\makebox(0,0)[r]{\strut{} 140}}%
      \put(792,2083){\makebox(0,0)[r]{\strut{} 160}}%
      \put(792,2411){\makebox(0,0)[r]{\strut{} 180}}%
      \put(792,2740){\makebox(0,0)[r]{\strut{} 200}}%
      \put(924,220){\makebox(0,0){\strut{} 0.84}}%
      \put(1302,220){\makebox(0,0){\strut{} 0.86}}%
      \put(1681,220){\makebox(0,0){\strut{} 0.88}}%
      \put(2059,220){\makebox(0,0){\strut{} 0.9}}%
      \put(2437,220){\makebox(0,0){\strut{} 0.92}}%
      \put(2815,220){\makebox(0,0){\strut{} 0.94}}%
      \put(3194,220){\makebox(0,0){\strut{} 0.96}}%
      \put(3572,220){\makebox(0,0){\strut{} 0.98}}%
      \put(2248,3070){\makebox(0,0){\strut{}comp15}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2585,2567){\makebox(0,0)[r]{\strut{}AMOSA}}%
      \csname LTb\endcsname%
      \put(2585,2347){\makebox(0,0)[r]{\strut{}known best solution}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{paper-gnuplottex-fig5}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> paper-gnuplottex-fig6.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(792,440){\makebox(0,0)[r]{\strut{} 50}}%
      \put(792,728){\makebox(0,0)[r]{\strut{} 100}}%
      \put(792,1015){\makebox(0,0)[r]{\strut{} 150}}%
      \put(792,1303){\makebox(0,0)[r]{\strut{} 200}}%
      \put(792,1590){\makebox(0,0)[r]{\strut{} 250}}%
      \put(792,1878){\makebox(0,0)[r]{\strut{} 300}}%
      \put(792,2165){\makebox(0,0)[r]{\strut{} 350}}%
      \put(792,2453){\makebox(0,0)[r]{\strut{} 400}}%
      \put(792,2740){\makebox(0,0)[r]{\strut{} 450}}%
      \put(924,220){\makebox(0,0){\strut{} 0.88}}%
      \put(1189,220){\makebox(0,0){\strut{} 0.89}}%
      \put(1454,220){\makebox(0,0){\strut{} 0.9}}%
      \put(1718,220){\makebox(0,0){\strut{} 0.91}}%
      \put(1983,220){\makebox(0,0){\strut{} 0.92}}%
      \put(2248,220){\makebox(0,0){\strut{} 0.93}}%
      \put(2513,220){\makebox(0,0){\strut{} 0.94}}%
      \put(2778,220){\makebox(0,0){\strut{} 0.95}}%
      \put(3042,220){\makebox(0,0){\strut{} 0.96}}%
      \put(3307,220){\makebox(0,0){\strut{} 0.97}}%
      \put(3572,220){\makebox(0,0){\strut{} 0.98}}%
      \put(2248,3070){\makebox(0,0){\strut{}comp21}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2585,2567){\makebox(0,0)[r]{\strut{}AMOSA}}%
      \csname LTb\endcsname%
      \put(2585,2347){\makebox(0,0)[r]{\strut{}known best solution}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{paper-gnuplottex-fig6}}%
    \gplfronttext
  \end{picture}%
\endgroup

